On Formal Feature Attribution and Its Approximation

Recent years have witnessed the widespread use of artificial intelligence (AI) algorithms and machine learning (ML) models. Despite their tremendous success, a number of vital problems like ML model brittleness, their fairness, and the lack of interpretability warrant the need for the active developments in explainable artificial intelligence (XAI) and formal ML model verification. The two major lines of work in XAI include feature selection methods, e.g. Anchors, and feature attribution techniques, e.g. LIME and SHAP. Despite their promise, most of the existing feature selection and attribution approaches are susceptible to a range of critical issues, including explanation unsoundness and out-of-distribution sampling. A recent formal approach to XAI (FXAI) although serving as an alternative to the above and free of these issues suffers from a few other limitations. For instance and besides the scalability limitation, the formal approach is unable to tackle the feature attribution problem. Additionally, a formal explanation despite being formally sound is typically quite large, which hampers its applicability in practical settings. Motivated by the above, this paper proposes a way to apply the apparatus of formal XAI to the case of feature attribution based on formal explanation enumeration. Formal feature attribution (FFA) is argued to be advantageous over the existing methods, both formal and non-formal. Given the practical complexity of the problem, the paper then proposes an efficient technique for approximating exact FFA. Finally, it offers experimental evidence of the effectiveness of the proposed approximate FFA in comparison to the existing feature attribution algorithms not only in terms of feature importance and but also in terms of their relative order.

==> approach.tex <==
\section{Decision Sets by Boosted Tree Compilation}\label{sec:cpl}

Based on~\cite{iisms-aaai22}, this section details a MaxSAT-based
approach to compiling a BT into a DS where each rule in the DS is
equivalent to the prime implicant of the BT classification function.

\input{rule}
\input{cmpl}
\input{phred}


==> relw.tex <==
\section{Related Work} \label{sec:relw}
%%
%Interpretable decision sets are logic-based ML models that can be
%traced back to 70s and
%80s~\cite{michalski-isip69,rivest-ipl76,breiman-bk84,rivest-ml87}.
%%
%To the best of our knowledge, \cite{clark-ewsl91} proposed the first
%approach to decision sets, which were introduced as the variant of
%decision lists~\cite{rivest-ml87,clark-ml89}.
%%
%The first method making use of logic and optimization to synthesize a
%disjunction of rules that match a given dataset was proposed
%in~\cite{resende-mp92}.
%%
%Recent work~\cite{leskovec-kdd16} argued that decision sets are more
%interpretable than the other logic-based models, i.e. decision lists
%and decision trees.
%%
%This work uses smooth local search to generate a set of rules first and heuristically minimizes a
%linear combination of criteria afterwards, e.g. the size of a rule,
%the maximum number of rules, the overlap or error of the rules.
%
%Since then a number of works proposed the use of logic reasoning and
%optimization procedures to train DS
%models~\cite{ipnms-ijcar18,meel-cp18,gm19,yisb-cp20,ilsms-aaai21}
%claiming to significantly outperform the approach
%of~\cite{leskovec-kdd16} in terms of accuracy and performance.
%%
%Among those, the works closest to ours
%are~\cite{ipnms-ijcar18,yisb-cp20,ilsms-aaai21}.
%%
%They proposed SAT-based approaches to computing smallest-size decision
%sets that \emph{perfectly} agree with the training data by minimizing
%either the number of rules~\cite{ipnms-ijcar18,ilsms-aaai21} or the
%number of literals~\cite{yisb-cp20,ilsms-aaai21} used in the model.
%%
%Additionally, \cite{yisb-cp20} is capable of computing \emph{sparse}
%decisions sets that trade off training accuracy for model size.
%%
%Despite the dramatic performance increase achieved
%in~\cite{ilsms-aaai21}, all the approaches above suffer from
%scalability issues.
%
%%
%%However, this approach is not as scalable as the SAT-based
%%approach~\cite{ipnms-ijcar18} to minimizing the number of rules,
%%which is shown to be more coarse-grained.
%%%
%%Moreover, \cite{yisb-cp20} proposed the sparse alternative trading
%%off its accuracy for smaller number of literals used to provide users
%%more succinct information.
%%
%% Motivated by the scalability limitations of the approaches above, of
%% perfectly accurate decision sets, \cite{ilsms-aaai21} proposed a novel
%% two-stage approach to the decision set computation problem, where the
%% method exhaustively enumerates individual rules and then computes a
%% subset of rules agreeing with the training data.
%
%%
%% Compared with the other work~\cite{yisb-cp20}, the exhaustive rule
%% enumeration process leads to a dramatically more compact encoding,
%% which contributes to a more scalable method of decision set generation
%% problems.
%%
%% The second part can be considered as a set cover problem, where the
%% authors minimize either the number of rules or the number of literals
%% in the model with the use of integer linear programming.
%%
%
%Post-hoc explainability is one of the major approaches to XAI.
%%
%Besides a plethora of heuristic sampling-based approaches to post-hoc
%explainability~\cite{guestrin-kdd16,lundberg-nips17,guestrin-aaai18},
%a formal reasoning based method to computing abductive
%explanations~\cite{darwiche-ijcai18,inms-aaai19} stands out.
%%
%AXps can be related with prime implicants of the decision function
%(hence an alternative name \emph{prime implicant explanations},
%\emph{PI-explanations}) associated with ML predictions and so are
%guaranteed to capture the semantics of the ML models in the entire
%feature space.
%%
%Although hard to compute in general, AXps were shown to be effectively
%computable for BT models by an incremental MaxSAT-based
%approach~\cite{iisms-aaai22}.
%
%Our work aims at making a bridge between interpretable DS models and
%AXp computation by exploiting the latter for training the former.
%%
%In particular and given a BT model, it focuses on generating decision
%rules that agree with the BT.
%%
%Each decision rule represents an AXp for the prediction made by the BT
%model, resulting in a DS model in a way \emph{guided} by the original
%BT model.
%%
%The approach is shown to outperform the prior logic-based approaches
%to DS inference in terms of test accuracy and performance.

